Gen6D: Generalizable Model-Free 6-DoF Object Pose Estimation from RGB Images

In this paper, we present a generalizable model-free 6-DoF object pose estimator called Gen6D. Existing generalizable pose estimators either need high-quality object models or require additional depth maps or object masks in test time, which significantly limits their application scope. In contrast, our pose estimator only requires some posed images of the unseen object and is able to accurately predict the poses of the object in arbitrary environments. Gen6D consists of an object detector, a viewpoint selector and a pose refiner, all of which do not require the 3D object model and can generalize to unseen objects. Experiments show that Gen6D achieves state-of-the-art results on two model-free datasets: the MOPED dataset and a new GenMOP dataset collected by us. In addition, on the LINEMOD dataset, Gen6D achieves competitive results compared with instance-specific pose estimators. Project page: https://liuyuan-pal.github.io/Gen6D/.

==> table/ab_data_linemod.tex <==
\begin{table}[]
    \centering
    \caption{Caption}
    \begin{tabular}{c C{0.08\linewidth} C{0.08\linewidth} C{0.08\linewidth}C{0.08\linewidth}C{0.08\linewidth}C{0.08\linewidth}}
    \toprule
    \multirow{2}{*}{Trainingset} & 
    \multicolumn{5}{c}{Object Name} & \multirow{2}{*}{Avg.}\\
    &  cat  & duck & bvise &  cam  & driller & \\
    Syn.+GMP+LM & 60.68 & 40.47 & 77.03 & 66.67 & 67.39 & \textbf{62.45} \\
    Syn.+GMP & 40.92 & 16.24 & 62.11 & 45.59 & 48.76 & 42.72 \\
    Syn.     & 31.04 & 11.64 & 61.63 & 35.39 & 54.61 & 38.86 \\
    \end{tabular}
    
    \label{tab:ab_data_linemod}
\end{table}
